A unifying evolutionary framework for infrared-selected obscured and unobscured quasar host haloes

Recent measurements of the dark matter halo masses of infrared-selected obscured quasars are in tension --- some indicate that obscured quasars have higher halo mass compared to their unobscured counterparts, while others find no difference. The former result is inconsistent with the simplest models of quasar unification that rely solely on viewing angle, while the latter may support such models. Here, using empirical relationships between dark matter halo and supermassive black hole masses, we provide a simple evolutionary picture that naturally explains these findings and is motivated by more sophisticated merger-driven quasar fueling models. The model tracks the growth rate of haloes, with the black hole growing in spurts of quasar activity in order to "catch-up" with the $M_{\textrm{BH}}$ - $M_{\textrm{star}}$ - $M_{\textrm{halo}}$ relationship. The first part of the quasar phase is obscured and is followed by an unobscured phase. Depending on the luminosity limit of the sample, driven by observational selection effects, a difference in halo masses may or may not be significant. For high luminosity samples, the difference can be large (a few to 10 times higher masses in obscured quasars), while for lower luminosity samples the halo mass difference is very small, much smaller than current observational constraints. Such a simple model provides a qualitative explanation for the higher mass haloes of obscured quasars, as well as rough quantitative agreement with seemingly disparate results.

==> commands_mnras.tex <==
% personal LaTex mark--ups
%
%
%        **** DO NOT MODIFY BELOW ****   **** DO NOT MODIFY BELOW ****
% Symbols
\newcommand{\cf}{C_{\mathrm{f}}}
\newcommand{\cc}{C_{\mathrm{c}}}
\newcommand{\celr}{C_{\mathrm{elr}}}
\newcommand{\tauc}{\tau_c}
\newcommand{\taue}{\tau_{\mathrm{elr}}}
\newcommand{\DR}{{\sc d.r.}}
\newcommand{\lambdarest}{\lambda_{\mathrm{o}}}
\newcommand{\lambdadop}{\Delta \lambda_{\mathrm{D}}}
\newcommand{\nulumnu}{\nu L_{\nu}}
\newcommand{\zabs}{z_{\mathrm{abs}}}
\newcommand{\zem}{z_{\mathrm{em}}}
\newcommand{\zsys}{z_{\mathrm{sys}}}
\newcommand{\aox}{\alpha_{\mathrm{ox}}}
\newcommand{\aopt}{\alpha_{\mathrm{o}}}
\newcommand{\arad}{\alpha_{\mathrm{r}}}
\newcommand{\axray}{\alpha_{\mathrm{x}}}
\newcommand{\mwind}{\dot{M}_{\mathrm{wind}}}
\newcommand{\macc}{\dot{M}_{\mathrm{acc}}}
\newcommand{\mfuel}{\dot{M}_{\mathrm{fuel}}}
\newcommand{\rew}{W_{\mathrm{r}}}
\newcommand{\ewlim}{W_{\mathrm{lim}}}
\newcommand{\NH}{N_\mathrm{H}}
%\newcommand{\bmath}[1]{\boldsymbol{#1}}
% Codes
\newcommand{\pimms}{\sc pimms}
\newcommand{\cloudy}{\sc cloudy}
% Units
\newcommand{\fwhm}{\sc fwhm}
\newcommand{\kms}{km~s$^{-1}$}
\newcommand{\percmsq}{cm$^{-2}$}
\newcommand{\lumunit}{\mathrm{erg~s}^{-1}}
\newcommand{\lumnuunit}{\mathrm{erg~s}^{-1}~\mathrm{Hz}^{-1}}
\newcommand{\fnuunit}{\mathrm{erg~cm}^{-2}~\mathrm{s}^{-1}~\mathrm{Hz}^{-1}}
%\newcommand{\arcdeg}{^{\circ}}
%\newcommand{\arcsec}{''}
\newcommand{\Msun}{M$_{\odot}$}
\newcommand{\rg}{R_\mathrm{g}}
% Journals
\newcommand{\apj}{ApJ}
\newcommand{\apjs}{ApJS}
\newcommand{\apjl}{ApJL}
\newcommand{\aj}{AJ}
\newcommand{\araa}{ARA\&A}
\newcommand{\aap}{A\&Ap}
\newcommand{\aaps}{A\&ApS}
\newcommand{\mnras}{MNRAS}
\newcommand{\iaucirc}{IAU Circular}
\newcommand{\jasa}{Journal of the American Statistical Association}
\newcommand{\jqsrt}{Journal of Quantitative Spectroscopy and Radiative Transfer}
\newcommand{\nat}{Nature}
\newcommand{\pasp}{PASP}
\newcommand{\etal}{et~al.}
\newcommand{\arxiv}{arXiv}

% Atomic stuff
\newcommand{\CIVdblt}{C\,{\sc iv}~$\lambda\lambda$1548, 1550}
\newcommand{\MgIIdblt}{Mg\,{\sc ii}~$\lambda\lambda$2796, 2803}
\newcommand{\AlIIIdblt}{Al\,{\sc iii}~$\lambda\lambda$1855, 1863}
\newcommand{\NVdblt}{N\,{\sc v}~$\lambda\lambda$1238, 1242}
\newcommand{\OVIdblt}{O\,{\sc vi}~$\lambda\lambda$1031, 1037}
\newcommand{\SiIIdblt}{Si\,{\sc ii}~$\lambda\lambda$1190, 1193}
\newcommand{\SiIVdblt}{Si\,{\sc iv}~$\lambda\lambda$1393, 1402}

\newcommand{\CIVw}{C\,{\sc iv}~$\lambda$1549}
\newcommand{\MgIIw}{Mg\,{\sc ii}~$\lambda$2798}
\newcommand{\Hbw}{H$\beta$~$\lambda$4861}

\newcommand{\CIV}{C\,{\sc iv}}
\newcommand{\MgII}{Mg\,{\sc ii}}
\newcommand{\Hb}{H$\beta$}

%
\newcommand{\AlI}{Al\,{\sc i}}
\newcommand{\AlII}{Al\,{\sc ii}}
\newcommand{\AlIII}{Al\,{\sc iii}}
\newcommand{\CII}{C\,{\sc ii}}
\newcommand{\CIIe}{C\,{\sc ii}$^*$}
\newcommand{\CIII}{C\,{\sc iii}]}
%\newcommand{\CIV}{C\,{\sc iv}}
\newcommand{\CaII}{Ca\,{\sc ii}}
\newcommand{\HI}{H\,{\sc i}}
\newcommand{\HII}{H\,{\sc ii}}
\newcommand{\HeI}{He\,{\sc i}}
\newcommand{\HeII}{He\,{\sc ii}}
\newcommand{\Lya}{Ly\,$\alpha$}
\newcommand{\Lyb}{Ly\,$\beta$}
\newcommand{\Lyg}{Ly\,$\gamma$}
%\newcommand{\Hb}{{H}\,$\beta$}
\newcommand{\FeII}{Fe\,{\sc ii}}
\newcommand{\FeIII}{Fe\,{\sc iii}}
%\newcommand{\MgII}{Mg\,{\sc ii}}
\newcommand{\MgX}{Mg\,{\sc x}}
\newcommand{\NI}{N\,{\sc i}}
\newcommand{\NIII}{N\,{\sc iii}}
\newcommand{\NV}{N\,{\sc v}}
\newcommand{\NaI}{Na\,{\sc i}}
\newcommand{\PV}{P\,{\sc v}}
\newcommand{\OI}{O\,{\sc i}}
\newcommand{\OII}{O\,{\sc ii}}
\newcommand{\OIII}{[O\,{\sc iii}]}
\newcommand{\OIIIsemi}{O\,{\sc iii}]}
\newcommand{\OVI}{O\,{\sc vi}}
\newcommand{\OVII}{O\,{\sc vii}}
\newcommand{\OVIII}{O\,{\sc viii}}
\newcommand{\SII}{S\,{\sc ii}}
\newcommand{\SiI}{Si\,{\sc i}}
\newcommand{\SiII}{Si\,{\sc ii}}
\newcommand{\SiIII}{Si\,{\sc iii}]}
\newcommand{\SiIV}{Si\,{\sc iv}}
\newcommand{\NeVIII}{Ne\,{\sc viii}}
\newcommand{\NiII}{Ni\,{\sc ii}}

\newcommand\ion[2]{#1$\;${\small\rmfamily\@Roman{#2}}\relax}%
%\newcommand\arcsec{\mbox{$^{\prime\prime}$}}%
%\newcommand\arcdeg{\mbox{$^\circ$}}%
%\newcommand{\rmn}[1]{{\mathrm{#1}}}

% Black hole mass stuff
\newcommand{\fwhmhb}{FWHM$(\textrm{H}\beta)$}
\newcommand{\fwhmciv}{FWHM$(\textrm{C\,{\sc iv}})$}
\newcommand{\fwhmmgii}{FWHM$(\textrm{Mg\,{\sc ii}})$}
\newcommand{\mbhhb}{M$_{BH}(\textrm{H}\beta)$}
\newcommand{\mbhciv}{M$_{BH}(\textrm{C\,{\sc iv}})$}
\newcommand{\mbhmgii}{M$_{BH}(\textrm{Mg\,{\sc ii}})$}
%\newcommand{\mbhhb}{M$_{\textrm{BH}}^{\textrm{H}\beta}$}
%\newcommand{\mbhciv}{M$_{\textrm{BH}}^{\textrm{C\,{\sc iv}}}$}
%\newcommand{\mbhmgii}{M$_{\textrm{BH}}^{\textrm{Mg\,{\sc ii}}}$}



%%
%% MACROS BELOW ARE NEEDED FOR BIOGRAPHICAL SKETCHES
%%
\def \pub {\par \hangindent = 2em \hangafter = 1 \noindent}
\def\lsim{\lower0.3em\hbox{$\,\buildrel <\over\sim\,$}}
\def\gsim{\lower0.3em\hbox{$\,\buildrel >\over\sim\,$}}
\def \etal{{\it et al.}}

%
%        **** DO NOT MODIFY ABOVE ****   **** DO NOT MODIFY ABOVE ****
%

